A Closer Look at Logical Reasoning with LLMs: The Choice of Tool Matters

The emergence of Large Language Models (LLMs) has demonstrated promising progress in solving logical reasoning tasks effectively. Several recent approaches have proposed to change the role of the LLM from the reasoner into a translator between natural language statements and symbolic representations which are then sent to external symbolic solvers to resolve. This paradigm has established the current state-of-the-art result in logical reasoning (i.e., deductive reasoning). However, it remains unclear whether the variance in performance of these approaches stems from the methodologies employed or the specific symbolic solvers utilized. There is a lack of consistent comparison between symbolic solvers and how they influence the overall reported performance. This is important, as each symbolic solver also has its own input symbolic language, presenting varying degrees of challenge in the translation process. To address this gap, we perform experiments on 3 deductive reasoning benchmarks with LLMs augmented with widely used symbolic solvers: Z3, Pyke, and Prover9. The tool-executable rates of symbolic translation generated by different LLMs exhibit a near 50% performance variation. This highlights a significant difference in performance rooted in very basic choices of tools. The almost linear correlation between the executable rate of translations and the accuracy of the outcomes from Prover9 highlight a strong alignment between LLMs ability to translate into Prover9 symbolic language, and the correctness of those translations.

==> logic.tex <==

\subsection{Formalism}
The study of logic and reasoning has been explored by philosophers for thousands of years. This paper focuses on two aspects of logical reasoning (1) translation of natural language to formal logic (i.e., how natural language is represented in logical reasoning tasks.) and (2) The tools used in the tool-based approach.
\subsection{Natural Language to Formal Logic}
Natural language is inherently ambiguous and context-dependent \cite{NLR_survey}. In contrast, formal logic is unambiguous and context-independent. It priorities logical consistency and prevents contradictions. The translation of NL to FOL is a brittle and error-prone process. The translations not only need to be structurally correct but also functional (i.e., symbolic solvers can properly process the translation without errors). Traditionally, NL-FOL translation has been addressed via rule-based methods \cite{classicalNL_FOL}, but they suffer from coverage issues and fail to scale to real-life applications. Therefore, attention has been placed on LLMs to solve the NL to FOL translation problem through instruction tuning and prompting LLMs \cite{NL-FOL,logicLM}. 

% Ehsan: fixed the notation errors for you
\paragraph{Propositional logic} also known as First-order Logic (FOL) is built around objects and relations. It has a simple paradigm consisting of combinations of seven fundamental logics (FOLs, including conjunction $\land$, disjunction $\lor$, negation $\neg$, implication $\rightarrow$, equation $ \equiv$, universal quantifier $\forall$, and existential quantifier $\exists$) with simple propositions \cite{MathLogic}. Symbolic solver's input language is constructed upon these fundamental logics, the distinction lies in their respective representations (e.g., Z3 uses Forall() instead of $\forall$. Pyke and Prover9 use the same FOL symbol $\forall$).

\begin{table}[t]
\centering
\begin{tabular}{|l|l|l|}
\hline
Dataset          & Synthetic & Reasoning Type \\ \hline
FOLIO            & \ding{55}     & FOL \\
ProofWriter       & \ding{51}     & Deductive      \\
PrOntoQA         & \ding{51}       & Deductive      \\
LogiQA           & \ding{51}      & Mixed          \\
CLUTTR           & \ding{51}      & Inductive      \\
BoardgameQA & \ding{51}       & Deductive      \\
LogicNLI         & \ding{51}       & Deductive      \\
AR-LSAT          & \ding{55}     & Analytical     \\ \hline
\end{tabular}
\caption{Statistic of typical datasets used for Natural Language Reasoning with LLMs.}
\label{Statistic of Typical Datasets for LLM NLR}
\end{table}
Table \ref{Statistic of Typical Datasets for LLM NLR} provides a summary of typical logical reasoning datasets used to evaluate the different types of logical reasoning capabilities of LLMs. 
\subsection{Logical Reasoning Tools}\label{tools}
\paragraph{Z3} is a satisfiability modulo theories (SMT) solver developed by Microsoft \cite{Z3}. The SMT solver provides algorithms to determine whether a set of mathematical formulas is satisfiable.  Z3 encompasses a diverse array of functionalities, including equality reasoning, arithmetic operations, manipulation of fixed-size bit-vectors, handling of arrays, and incorporation of quantifiers. More importantly, Z3 is also a theorem prover for first-order logic augmented with various built-in theories \cite{DKAL}. These capabilities make Z3 a versatile tool for a wide range of applications in research. 

As shown in Table \ref{Tool Summary Table}, recent studies have tackled a wide range of logical reasoning datasets using Z3 incorporated with LLMs.
 As demonstrated in Appendix \ref{Z3 ProofWriter Prompts}, Z3's required translation from LLM is sentence by sentence, eliminating the need for pre-defining predicates, facts, and queries as required in Pyke. This capability simplifies the process for LLMs to interpret and implement Z3. In addition, Z3 is more dynamic than Prover9 and Pyke. For example, Z3 is the only symbolic solver that supports setting preferences over different rules (i.e., rule 2 is preferred over rule 5) as shown in \citet{satlm}. This is because Z3 directly uses Python as its main programming language, the execution of Z3 does not require extra files or a specific programming language. An example of how Z3 tackles BordgameQA is included in Appendix \ref{BoardgameQA Z3}. Because Z3 was developed as an SMT solver which focuses on analytical reasoning, it has been underutilised for solving deductive and FOL problems. \citet{satlm} is the only study incorporating Z3 in solving deductive reasoning problems.
\paragraph{Pyke} is a theorem solver with a Python-based framework used for building and executing rule-based expert systems. \cite{Pyke}.  Pyke uses a backward-chaining rule-based system, similar to Prolog \cite{Prolog}, to generate a function call graph before the functions are called. Given a logical question, Pyke initially establishes a knowledge base and incorporates all known Facts and Rules from the solver’s inputs. Then, it iteratively applies given Rules on already known Facts, aiming at obtaining more implied Facts until the conclusion is proved or disproved. The reasoning process of Pyke is a black box but \citet{logical_solver} modified Pyke's source code and trained LLM's on it to solve logical reasoning tasks. This approach yielded promising outcomes, demonstrating the adaptability and effectiveness of Pyke in facilitating logical inference tasks. Compared to Z3, Pyke was specifically built for solving FOL reasoning tasks, and the conclusions do not require extra programming (i.e., Conclusions are automatically True/False/Unknown, whereas Z3 requires extra rule setting for Unknown conclusions because it can only produce Satisfiable or Unsatisfiable results). However, Pyke's language is less dynamic, and the execution requires extra files (i.e., need to pre-define rule.krb, fact.krb and query.krb files) which makes the logical reasoning task translation more error-prone. Furthermore, Pyke presents challenges in installation and is susceptible to capacity limitations in different operating systems.
\paragraph{Prover9} is an automated theorem prover for first-order and equational logic based on resolution \cite{resolution} and paramodulation rules.  Prover9 converts FOL statements to conjunctive normal form (CNF) and then performs resolution on the CNF to deduce whether a conclusion is true, false, or unknown. Prover9 is less flexible compared to Z3 because it is not a Python package and does not support a variety of dynamic operations like setting rule preferences. Prover9 uses FOL as its programming language, simplifying the task since LLMs like GPT \cite{gpt3} are proficient with NL-FOL translations. In addition, Prover9's package can be installed online, but like Pyke, it is susceptible to capacity limitations in different operating systems.

==> tools.tex <==
\begin{table}[t]
\centering
\scalebox{0.85}{
\begin{tabular}{lccc}
\hline
  & \texttt{Proofwriter} & \texttt{FOLIO} & \texttt{ProntoQA}\\
\hline
Base &  &  &   \\
Z3    &  &  &  \\
Prover9  &  &  &  \\
Pyke   &  &  &  \\
\hline
\end{tabular}}
\caption{Results of 2-shot ......}
\label{table:tool_results}
\end{table}

\subsection{Formalisms for Logical Reasoning}

\paragraph{First Order Logic.}

\paragraph{Integer Linear Program.}


\subsection{SMT or SAT Solvers}
\paragraph{Z3.} ...

\paragraph{Pyke.} ...

\paragraph{Prover9.} ...

Maybe some sort of a table where you summarize the key differences between these tools.
